Minimal Submanifolds and Waists of Locally Symmetric Spaces

We study the higher expansion properties of locally symmetric spaces, with a particular focus on octonionic hyperbolic manifolds. We show that codimension two minimal submanifolds of compact octonionic locally symmetric spaces must have large volume, at least linear in the volume of the ambient space. As a corollary we prove linear waist inequalities for octonionic hyperbolic manifolds in codimension two and construct the first locally symmetric examples of power-law systolic freedom. We also show that any codimension two submanifold of small volume can be homotoped to a lower dimensional set. We use this to prove that branched covers of octonionic hyperbolic manifolds are stable in the sense of Dinur-Meshulam and to establish a uniform lower bound on the non-abelian Cheeger constants of octonionic hyperbolic manifolds. In a more general setting, we prove that maps from locally symmetric spaces to low dimensional euclidean spaces admit fibers whose fundamental group has large exponent of growth. We show as a consequence that cocompact lattices in $SL_n(\mathbb{R})$ have property $ FA_{\lfloor n/8\rfloor-1}$: any action on a contractible $CAT(0)$ simplicial complex of dimension at most $ \lfloor n/8\rfloor -1$ has a global fixed point.

==> LetterDrafts/Comments/comments.tex <==
Hee Oh:
- Burger-Roblin density is a bad name (fixed)
- Add citation to the matric coeff paper (done)

==> LetterDrafts/Dinuremail.tex <==
Dear Irit,

With Ben Lowe we recently finished a paper "Minimal Submanifolds and Waists of Locally Symmetric Spaces", the most updated version is here: https://drive.google.com/file/d/1ncPMlEPgtJEW65ajeq2VLqdzOMwcWqda/view?usp=sharing.

We use minimal surfaces to prove various results on octonionic hyperbolic manifolds which have "higher expansion flavor". In particular, we prove that triangulations of these manifolds satisfy cover stability in the sense of your paper with Roy Meshulam. We also show that small cycles in low codimensions can be efficiently homotoped to lower dimension. We're both a little distant from the higher expansion area so we'd be very grateful if let us know if there is any recent development and papers we should be aware of, as well as any other comments and question you might have.

Best,
Mikolaj and Ben


==> LetterDrafts/Heeemail.tex <==
Dear Hee, 

With Ben Lowe we recently finished a paper "Minimal Submanifolds and Waists of Locally Symmetric Spaces", the most updated version is here: https://drive.google.com/file/d/1ncPMlEPgtJEW65ajeq2VLqdzOMwcWqda/view?usp=sharing.

One of the most important ingredients in our proofs are your bounds on the decay of matrix coefficient and the resulting growth gaps. We use them to show that actions of some higher rank lattices on low dimensional CAT(0) complexes have a fixed point. It is related to the project on minimal submanifolds I mentioned to you when I visited Yale few years ago.

We'd be grateful for any comments or questions.  

Best,
Mikolaj and Ben


==> LetterDrafts/MeshulamEmail.tex <==
Dear Roy,

With Ben Lowe we recently finished a paper "Minimal Submanifolds and Waists of Locally Symmetric Spaces", the most updated version is here: https://drive.google.com/file/d/1ncPMlEPgtJEW65ajeq2VLqdzOMwcWqda/view?usp=sharing.

We use minimal surfaces to prove various results on octonionic hyperbolic manifolds which have "higher expansion flavor". In particular, we prove that triangulations of these manifolds satisfy cover stability in the sense of your paper with Irit Dinur. We also show that small cycles in low codimensions can be efficiently homotoped to lower dimension. We're both a little distant from the higher expansion area so we'd be very grateful if let us know if there is any recent development and papers we should be aware of, as well as any other comments and question you might have. 

Best,
Mikolaj and Ben


==> LetterDrafts/RomanUri.tex <==
Dear Roman and Uri,

With Ben Lowe we recently completed a paper "Minimal Submanifolds and Waists of Locally Symmetric Spaces", the most updated version is here: https://drive.google.com/file/d/1ncPMlEPgtJEW65ajeq2VLqdzOMwcWqda/view?usp=sharing.

One of the things we prove is a linear waist inequality in codimension 2 for octonionic hyperbolic manifolds. We cite your paper for the generalization to covers of manifolds with Kazhdan fundamental group and try to hint the differences between our approaches at the end of Section 1.1, please let us know if we should change anything.

We'd be grateful for any comments or questions.  

Best,
Mikolaj and Ben

==> LetterDrafts/Tsachikemail.tex <==
Dear Tsachik,

With Ben Lowe we recently completed a paper "Minimal Submanifolds and Waists of Locally Symmetric Spaces", the most updated version is here: https://drive.google.com/file/d/1ncPMlEPgtJEW65ajeq2VLqdzOMwcWqda/view?usp=sharing.

The paper is studying higher expansion properties of locally symmetric spaces, with a particular focus on octonionic hyperbolic manifolds. In particular, we show that a branched cover of such a manifold with a small branching locus can be "cheaply" cut and reconnected to form a true cover. This still not enough for flexible stability but hopefully goes in the right direction. 

We'd be grateful for any comments or questions. 

Best,
Mikolaj and Ben

==> LetterDrafts/acknowledgements.tex <==
We are grateful to Larry Guth for bringing to our attention the work by Alagalingam.  We are grateful to Benson Farb for a helpful discussion regarding property $FA_r$.  We also thank Yangyang Li.

other people: -Shmuel - 

==> LetterDrafts/bensonemail.tex <==
Dear Benson,

With Mikolaj Fraczyk we recently completed a paper "Minimal Submanifolds and Waists of Locally Symmetric Spaces", the most updated version is here: https://drive.google.com/file/d/1ncPMlEPgtJEW65ajeq2VLqdzOMwcWqda/view?usp=sharing.  I told you about some of this two summers ago.  One thing we're doing that you might be interested in is establishing property FA_r for cocompact lattices in SL(n,R), for a linear in n range of dimensions r.  We also wanted to send it to you because the paper you wrote with Connell and McReynolds was the initial inspiration for our work.  

We'd be grateful for any comments or questions.  

Best,
Ben and Mikolaj

==> LetterDrafts/connellandfriends.tex <==
Dear Chris, Ben, and Shi,

With Mikolaj Fraczyk we recently completed a paper "Minimal Submanifolds and Waists of Locally Symmetric Spaces", the most updated version is here https://drive.google.com/file/d/1ncPMlEPgtJEW65ajeq2VLqdzOMwcWqda/view?usp=sharing.    We wanted to send it to you because we are using your natural flows in an important way, especially in the results described in 1.2 and 1.3 of the intro.   

One thing we comment on in relation to your work is that the cohomology vanishing you prove for infinite volume locally symmetric spaces holds in a linear-in-rank range of dimensions in the SL(n,R) case (I believe you already state this explicitly in your paper in the Anosov case.)  We put a comment to this effect in remark 1.23.  This came out of the computations we were doing to establish property FA_r for uniform lattices in SL(n,R) for a linear-in-n range of dimensions r (that isometric simpicial actions of lattices in SL(n,R) on r-dimensional nonpositively curved simplicial complexes have global fixed points.)  

We'd be grateful for any comments or questions.

Best,
Ben and Mikolaj

==> LetterDrafts/fernandocodaemail.tex <==
 "Minimal Submanifolds and Waists of Locally Symmetric Spaces", the most updated version is here: https://drive.google.com/file/d/1ncPMlEPgtJEW65ajeq2VLqdzOMwcWqda/view?usp=sharing

We are applying min-max and minimal surface theory to some problems about higher expansion properties of locally symmetric spaces, and then also using representation theory to say things about minimal submanifolds of low codimension.   

 We'd be grateful for any comments or questions.  

Best,
Ben and Mikolaj

==> LetterDrafts/guthemail.tex <==
Dear Larry,

With Mikolaj Fraczyk we recently completed a paper "Minimal Submanifolds and Waists of Locally Symmetric Spaces", the most updated version is here: https://drive.google.com/file/d/1ncPMlEPgtJEW65ajeq2VLqdzOMwcWqda/view?usp=sharing.  

Earlier in an email you told me about Alagalingam's paper, and we comment on how we can recover some of the results of that paper using our methods (this is on pg. 5 and 13.) 

We'd be grateful for any comments or questions.  

Best,
Ben 

==> LetterDrafts/lubotzkyemail.tex <==
Dear Alex,

With Ben Lowe we recently finished a paper "Minimal Submanifolds and Waists of Locally Symmetric Spaces", the most updated version is here: https://drive.google.com/file/d/1ncPMlEPgtJEW65ajeq2VLqdzOMwcWqda/view?usp=sharing.

We prove various results on the octonionic hyperbolic manifolds which have "higher expansion flavor". In particular, we prove that triangulations of these manifolds satisfy cover stability in the sense of Dinur-Meshulam (or section 4.4 of your paper with Michael Chapman). We also show that small cycles in low codimensions can be efficiently homotoped to lower dimension. We're both a little distant from the higher expansion area so we'd be very grateful if let us know if there is any recent development and papers we should be aware of, as well as any other comments and question you might have.

Best,
Mikolaj and Ben



==> LetterDrafts/minjuemail.tex <==
Dear Minju, 

With Mikolaj we recently finished a paper "Minimal Submanifolds and Waists of Locally Symmetric Spaces", the most updated version is here: https://drive.google.com/file/d/1ncPMlEPgtJEW65ajeq2VLqdzOMwcWqda/view?usp=sharing.

One of the most important ingredient in our proofs are your bounds on the decay of matrix coefficient and the resulting growth gaps. We use them to show that actions of some higher rank lattices on low dimensional CAT(0) complexes have a fixed point.

We'd be grateful for any comments or questions.  

Best,
Ben

==> LetterDrafts/sarnakemail.tex <==
Dear Peter,

With Mikolaj Fraczyk we recently completed a paper "Minimal Submanifolds and Waists of Locally Symmetric Spaces", the most updated version is here: https://drive.google.com/file/d/1ncPMlEPgtJEW65ajeq2VLqdzOMwcWqda/view?usp=sharing.

The paper is studying higher expansion properties of locally symmetric
spaces, with a particular focus on octonionic hyperbolic manifolds. Our approach is based on bringing new techniques into the picture from minimal surface theory and representation theory to study these problems.

Best,
Ben and Mikolaj

==> LetterDrafts/sendlist.tex <==
UChicago: (*-pre arxiv)

%Shumel*
%Benson*
Simion BL? 
%Minju*
%Andre 
Yangyang (can tell in person)
Karen (can tell in person) 
May BL 
Corlette BL?

Yale

Sebastian
%Hee* 
Dongrul Kim
Margulis
Yair Minsky BL

IAS/Princeton

%Irit Dinur*
%Peter Sarnak*
Asaf Naor BL? 
Anshul Adve BL 
Akshay Venkatesh
%Fernando 

MIT  
%Larry Guth*
%Jonathan Zung 
%Elia Portnoy 

Other places:
%Alex Lubtozky*,
Michael Chapman
Michael Freedman BL
Michael Hastings BL
%Roy Mashulam*,
Lewis Bowen,
%Roman Sauer* 
%Uri Bader* 
%Alex Furman 
%Tsachik Gelander*
Arie Levit 
Nir Lazarovich 
%David Fisher* 
% McReynolds
% Connell
Kapovich  BL?  
Yehuda Shalom 
Tom Hutchcroft
%Antoine Song
Gromov BL?
Shai Evra 
Tali Kaufman 
Sam Edwards
% Shi Wang
Yuping Ruan BL
Homin Lee BL
Itamar Vigdorovich
Burger BL?
Belolipetsky BL?
Harvey BL?
Lawson BL? 
Alon Dogon
Miklos Abert
Jean Raimbault
Emmanuel Breuillard
J.F. Quint 
Yves Beoist
Fanny Kassel
Delaunay triangulation authors
Ursula Hammenstadt BL?
%frieter jaekel
Robert Young
Martin Bridson 
Aaron Brown BL? 
Piotr Nowak
Piotr Mizerka 
Dawid Kielak 
Marc Lackenby
Grigori Avramidi 
Kevin Schreve
Boris Okun
Ralph Spatzier BL












==> LetterDrafts/shmuelemail.tex <==
Dear Shmuel,

We have just completed our paper with Ben: "Minimal submanifolds and waist of locally symmetric spaces". The most updated version is here: https://drive.google.com/file/d/1ncPMlEPgtJEW65ajeq2VLqdzOMwcWqda/view?usp=sharing.

I gave a talk about it at your birthday conference in New York. The results evolved a little bit. We omit the quaternionic case but on positive side we added a branched cover stability theorem for octonionic hyperbolic manifolds. 

One of our Theorems (1.6) shows that in codimensions 1 and 2 the absolute systoles of compact octonionic hyperbolic manifolds are linear in the volume. We also show that any small cycle in these codimensions can be efficiently homotoped to lower dimension, so that the image of the homotopy has area bounded linearly in terms of the area of the cycle. 

We'd be grateful for any comments or questions. 

Best,
Mikolaj and Ben
